First measurement of jet mass in Pb-Pb and p-Pb collisions at the LHC

This letter presents the first measurement of jet mass in Pb-Pb and p-Pb collisions at $\sqrt{s_{\rm NN}}$ = 2.76 TeV and 5.02 TeV, respectively. Both the jet energy and the jet mass are expected to be sensitive to jet quenching in the hot Quantum Chromodynamics (QCD) matter created in nuclear collisions at collider energies. Jets are reconstructed from charged particles using the anti-$k_{\rm T}$ jet algorithm and resolution parameter $R = 0.4$. The jets are measured in the pseudorapidity range $|\eta_{\rm{jet}}|<0.5$ and in three intervals of transverse momentum between 60 GeV/$c$ and 120 GeV/$c$. The measurement of the jet mass in central Pb-Pb collisions is compared to the jet mass as measured in p-Pb reference collisions, to vacuum event generators, and to models including jet quenching. It is observed that the jet mass in central Pb-Pb collisions is consistent within uncertainties with p-Pb reference measurements. Furthermore, the measured jet mass in Pb-Pb collisions is not reproduced by the quenching models considered in this letter and is found to be consistent with PYTHIA expectations within systematic uncertainties.

==> summary.tex <==
\newpage
\section{Summary}\label{sec:summary}
The ALICE collaboration measured the jet mass in minimum bias \pPb{} and 10\% most central \PbPb{} collisions. The fully corrected results were compared to event generators. JEWEL and QPYTHIA, event generators incorporating jet quenching, underestimate and overesimate the measured jet mass. The jet mass in PYTHIA, without modelling of hot QCD matter effects, is consistent with the measurement in \PbPb{} collisions.


